Red Teaming Program Repair Agents: When Correct Patches can Hide Vulnerabilities

LLM-based agents are increasingly deployed for software maintenance tasks such as automated program repair (APR). APR agents automatically fetch GitHub issues and use backend LLMs to generate patches that fix the reported bugs. However, existing work primarily focuses on the functional correctness of APR-generated patches, whether they pass hidden or regression tests, while largely ignoring potential security risks. Given the openness of platforms like GitHub, where any user can raise issues and participate in discussions, an important question arises: Can an adversarial user submit a valid issue on GitHub that misleads an LLM-based agent into generating a functionally correct but vulnerable patch? To answer this question, we propose SWExploit, which generates adversarial issue statements designed to make APR agents produce patches that are functionally correct yet vulnerable. SWExploit operates in three main steps: (1) program analysis to identify potential injection points for vulnerable payloads; (2) adversarial issue generation to provide misleading reproduction and error information while preserving the original issue semantics; and (3) iterative refinement of the adversarial issue statements based on the outputs of the APR agents. Empirical evaluation on three agent pipelines and five backend LLMs shows that SWExploit can produce patches that are both functionally correct and vulnerable (the attack success rate on the correct patch could reach 0.91, whereas the baseline ASRs are all below 0.20). Based on our evaluation, we are the first to challenge the traditional assumption that a patch passing all tests is inherently reliable and secure, highlighting critical limitations in the current evaluation paradigm for APR agents.

==> Alg/alg.tex <==
\section{Attack Algorithm}

\begin{wrapfigure}[19]{r}{0.54\textwidth}
\vspace{-0.3cm}
\begin{minipage}{0.54\textwidth}
\begin{algorithm}[H]
\caption{\algname Inference Pipeline}
\begin{algorithmic}[1]
\Require Safety policy set $\mathbb{P} = \{\pi_1, \cdots, \pi_n\}$, input video $\mathbf{v}$, query $q$, guardrail model $\mathcal{G}$, video encoder $\phi$, pruning parameter $K$, safety-aware frame sampler $\mathcal{S}$
\Ensure Guardrail flags $\{c_i \in \{0, 1\} \mid i \in [1, n]\}$, explanation $T_{\text{exp}}$
\State Sample frames from $\mathbf{v}$: $\{f_1, \cdots, f_{N_{\text{event}}}\} \leftarrow \mathcal{S}(\mathbf{v})$
\State Extract embeddings for each frame: $\mathbf{E}_i \leftarrow \phi(f_i)$ and concatenate as visual tokens $\mathcal{V}$ {\hspace{-0.2cm}\Comment{\color{blue} \eqnref{eqn:video_embedding}}}

\State Apply PEPE to encode policy chunks  {\Comment{\color{blue} \eqnref{eqn:pepe_attention}}}

\For{each policy $\pi_i \in \mathbb{P}$}  {\Comment{\color{blue} PAP}}
    \State Compute cross-attention score $r_i^j$ {\Comment{\color{blue} \eqnref{eqn:relevance_score_pair}}}
    \State Calculate policy-video relevance $r_i$ {\Comment{\color{blue} \eqnref{eqn:relevance_score}}}
    \State Select top-$k$ visual tokens: $\mathcal{V}^*_{\pi_i}$ {\Comment{\color{blue} \eqnref{eqn:top_k}}}
\EndFor
\State Update KV cache and discard pruned features
% \State Compute attention matrix $A^\mathbb{P}$ {\Comment{\color{blue} \eqnref{eqn:pepe_attention}}}
\State Decode guardrail flags and explanations {\Comment{\color{blue} \eqnref{eqn:guardrail_task}}}
\end{algorithmic}
\label{algo:guardrail}
\end{algorithm}
\end{minipage}
\end{wrapfigure}

==> Table/fun_asr.tex <==
% Table generated by Excel2LaTeX from sheet 'asr'
\begin{table}[htbp]
  \centering
  \caption{Add caption}
  \resizebox{0.98\textwidth}{!}{
    \begin{NiceTabular}{llcccccccccc}
    \CodeBefore
        \rowcolors{3}{}{blue!08}
        \Body
    \toprule
    \toprule
    \multicolumn{1}{r}{\multirow{2}[2]{*}{\textbf{Metric}}} & \multirow{2}[2]{*}{\textbf{Method}} & \multicolumn{5}{c}{\textbf{MINI}}     & \multicolumn{5}{c}{\textbf{SWE}} \\
          &       & \textbf{C-3.5-S} & \textbf{C-3.7-S} & \textbf{C-4.0-S} & \textbf{G-2.5-P} & \textbf{G-2.0-F} & \textbf{C-3.5-S} & \textbf{C-3.7-S} & \textbf{C-4.0-S} & \textbf{G-2.5-P} & \textbf{G-2.0-F} \\
    \midrule
    \multicolumn{1}{r}{\multirow{4}[2]{*}{\textbf{Pass@1}}} & \textbf{No-Attack} & \textbf{0.17} & \textbf{0.42} & \textbf{0.48} & \textbf{0.40} & \textbf{0.11} & \textbf{0.26} & \textbf{0.41} & \textbf{0.46} & \textbf{0.33} & \textbf{0.16} \\
          & \textbf{BugInject} & 0.10  & 0.32  & 0.34  & 0.34  & 0.06  & 0.13  & 0.21  & 0.27  & 0.31  & 0.09 \\
          & \textbf{AutoRed} & 0.07  & 0.30  & 0.21  & 0.11  & 0.07  & 0.02  & 0.07  & 0.01  & 0.17  & 0.10 \\
          & \textbf{Ours} & 0.17  & 0.41  & 0.48  & 0.30  & 0.11  & 0.16  & 0.32  & 0.45  & 0.30  & 0.10 \\
    \midrule
    \multicolumn{1}{r}{\multirow{3}[1]{*}{\textbf{ASR}}} & \textbf{BugInject} & 0.01  & 0.01  & 0.03  & 0.06  & 0.03  & 0.02  & 0.06  & 0.07  & 0.05  & 0.03 \\
          & \textbf{AutoRed} & 0.07  & 0.01  & 0.00  & 0.01  & 0.02  & 0.07  & 0.01  & 0.00  & 0.01  & 0.02 \\
          & \textbf{Ours} & \textbf{0.78} & \textbf{0.77} & \textbf{0.79} & \textbf{0.79} & \textbf{0.73} & \textbf{0.78} & \textbf{0.78} & \textbf{0.83} & \textbf{0.77} & \textbf{0.73} \\
    \multicolumn{1}{r}{\multirow{3}[1]{*}{\textbf{Correct-ASR}}} & \textbf{BugInject} & 0.02  & 0.04  & 0.01  & 0.01  & 0.02  & 0.03  & 0.02  & 0.05  & 0.06  & 0.07 \\
          & \textbf{AutoRed} & 0.04  & 0.01  & 0.08  & 0.20  & 0.09  & 0.04  & 0.01  & 0.08  & 0.20  & 0.09 \\
          & \textbf{Ours} & \textbf{0.75} & \textbf{0.80} & \textbf{0.78} & \textbf{0.74} & \textbf{0.91} & \textbf{0.82} & \textbf{0.82} & \textbf{0.87} & \textbf{0.75} & \textbf{0.84} \\
    \bottomrule
    \bottomrule
    \end{NiceTabular}%
    }
  \label{tab:addlabel}%
\end{table}%


==> Table/functionality.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Functionality Results }
  \resizebox{0.66\textwidth}{!}{
    \begin{NiceTabular}{llcccc}
    \CodeBefore
        \rowcolors{3}{}{blue!08}
        \Body
    \toprule
    \toprule
    \multirow{2}[2]{*}{\textbf{Agent}} & \multirow{2}[2]{*}{\textbf{LLM}} & \multicolumn{4}{c}{\textbf{Pass@1}} \\
          &       & \textbf{No-Attack} & \multicolumn{1}{l}{\textbf{BugInject}} & \multicolumn{1}{l}{\textbf{AutoRed}} & \multicolumn{1}{l}{\textbf{Ours}} \\
    \midrule
    \multirow{5}[1]{*}{\textbf{MINI}} & \textbf{Claude-3.5} & \textbf{0.17} & 0.10 (57.7) & 0.07 (40.4) & 0.17 (100) \\
          & \textbf{Claude-3.7} & \textbf{0.42} & 0.32 (76.8) & 0.3 (72.0) & 0.41 (98.4) \\
          & \textbf{Claude-4.0} & \textbf{0.48} & 0.34 (70.3) & 0.21 (43.4) & 0.48 (100) \\
          & \textbf{Gemini-2.5-pro} & \textbf{0.40} & 0.34 (84.3) & 0.11 (27.3) & 0.30 (74.4) \\
          & \textbf{Gemini-2.0-flash} & \textbf{0.11} & 0.06 (54.5) & 0.07 (63.6) & 0.11 (100) \\ \midrule
    \multirow{5}[0]{*}{\textbf{SWE}} & \textbf{Claude-3.5} & \textbf{0.26} & 0.13 (50.6) & 0.02 (7.8) & 0.16 (62.3) \\
          & \textbf{Claude-3.7} & \textbf{0.41} & 0.21 (51.2) & 0.07 (17.1) & 0.32 (78.0) \\
          & \textbf{Claude-4.0} & \textbf{0.46} & 0.27 (58.3) & 0.01 (2.2) & 0.45 (96.4) \\
          & \textbf{Gemini-2.5-pro} & \textbf{0.33} & 0.31 (94.9) & 0.17 (52.0) & 0.30 (92.8) \\
          & \textbf{Gemini-2.0-flash} & \textbf{0.16} & 0.09 (55.1) & 0.1 (61.2) & 0.10 (63.2) \\
          \bottomrule
          \bottomrule
    \end{NiceTabular}%
    }
  \label{tab:main}%
\end{table}%


==> Text/statement.tex <==

\section*{Impact Statements}


% \section* {Ethics Statement}
% This work adheres to the ICLR Code of Ethics. No human subjects or animal experimentation were involved. All datasets used, including SWE-Bench-Lite, were obtained in compliance with relevant usage guidelines, ensuring no privacy violations. We have carefully avoided biases or discriminatory outcomes. No personally identifiable information was used, and no experiments posed privacy or security risks. We are committed to transparency and integrity throughout the research process.

% \section* {Reproducibility Statement}
% We have taken steps to ensure that the results presented in this paper are reproducible. All code and datasets are publicly available in an anonymous repository to facilitate replication. The experimental setup is described in detail. 

% Furthermore, the public datasets used, such as SWE-Bench-Lite, are openly accessible, ensuring consistent and reproducible evaluation. These measures aim to enable other researchers to replicate our work and advance the field.

% \section* {LLM Usage}
% Large Language Models (LLMs) were employed solely to assist in writing and polishing the manuscript, including refining language, improving readability, and enhancing clarity. The LLM was used for tasks such as sentence rephrasing, grammar checking, and improving overall flow.

% The LLM was not involved in ideation, research methodology, or experimental design. All research concepts, analyses, and results were developed and conducted by the authors. The authors take full responsibility for the manuscript content, including any text generated or polished by the LLM, and confirm that all LLM-assisted text adheres to ethical guidelines and does not constitute plagiarism or scientific misconduct.

This paper studies the security implications of LLM–based automated program repair (APR) agents, and introduces a red-teaming methodology to expose a previously underexplored vulnerability: the generation of functionally correct yet exploitable patches under realistic CI/CD workflows. The primary goal of this work is to advance the robustness and safety of machine-learning–driven software engineering systems by identifying concrete failure modes that are not captured by existing evaluation paradigms.
\paragraph{Potential Risks and Misuse.}
Our work demonstrates that adversaries can exploit natural and legitimate interfaces—such as issue reports in open-source repositories—to induce APR agents to introduce hidden vulnerabilities. While the techniques presented could theoretically be misused to assist malicious actors, we emphasize that the threat model we study already exists in real-world deployments, independent of this paper. We do not release automated exploit-generation tools, real-world attack payloads, or end-to-end exploitation frameworks, and our experiments are conducted in controlled environments with benign proof-of-concept payloads. We believe that withholding analysis of such risks would create a false sense of security rather than prevent misuse.

\paragraph{Positive Societal Impact.}
By revealing that passing all regression tests is insufficient to guarantee the security of LLM-generated patches, this work highlights an important gap in current software maintenance practices. Our findings encourage the development of security-aware evaluation metrics, branch-coverage–aware testing, and adversarially robust APR pipelines. In the long term, this can contribute to more trustworthy software supply chains, safer deployment of autonomous coding agents, and improved security practices in open-source ecosystems that increasingly rely on automation.

\paragraph{Ethical Considerations.}
We view this work as defensive in nature. The intent is not to enable attacks, but to provide empirical evidence that motivates stronger safeguards before APR agents are more widely deployed in safety-critical or security-sensitive contexts. All vulnerabilities studied are standard, well-documented CWEs, and no proprietary systems or private repositories are targeted. We hope this work will inform both researchers and practitioners about the necessity of integrating security considerations into the design, evaluation, and governance of machine-learning–based software engineering tools.

Overall, we believe that the benefits of exposing and understanding these risks outweigh the potential harms, and that this work supports the responsible development and deployment of autonomous program repair systems.


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

